Rational curves on genus one fibrations

In this paper we look for necessary and sufficient conditions for a genus one fibration to have rational curves. We show that a projective variety with log terminal singularities that admits a relatively minimal genus one fibration $X\rightarrow B$ does contain vertical rational curves if and only if it not isomorphic to a finite \'etale quotient of a product $\tilde{B}\times E$ over $B$. Many sufficient conditions for the existence of rational curves in a variety that admits a genus one fibration are proved in this paper.

==> enunciato.tex <==
\begin{theorem}\label{maintheorem}
	Let $(X,\Delta)$ be a klt pair such that there exists a surjective morphism $\phi:X\rightarrow B$ to a variety of dimension $n-1$. Suppose moreover $K_X+\Delta \equiv_{\text{num}} \phi^*L$ for some $\Q $-divisor on $B$ and the augmented irregularity of $X$ is zero, then there exists a subvariety of $X$ covered by rational curves contracted by $\phi$.
\end{theorem}
